A Note on Quantum Phase Estimation

In this work, we study the phase estimation problem. We show an alternative, simpler and self-contained proof of query lower bounds. Technically, compared to the previous proofs [NW99, Bes05], our proof is considerably elementary. Specifically, our proof consists of basic linear algebra without using the knowledge of Boolean function analysis and adversary methods. Qualitatively, our bound is tight in the low success probability regime and offers a more fine-grained trade-off. In particular, we prove that for any $\epsilon > 0, p \geq 0$, every algorithm requires at least $\Omega(p/{\epsilon})$ queries to obtain an ${\epsilon}$-approximation for the phase with probability at least p. However, the existing bounds hold only when $p > 1/2$. Quantitatively, our bound is tight since it matches the well-known phase estimation algorithm of Cleve, Ekert, Macchiavello, and Mosca [CEMM98] which requires $O(1/{\epsilon})$ queries to obtain an ${\epsilon}$-approximation with a constant probability. Following the derivation of the lower bound in our framework, we give a new and intuitive interpretation of the phase estimation algorithm of [CEMM98], which might be of independent interest.

==> TODO.tex <==
Parallel vs sequential: Hadamard test

Add Table including upper bounds: Xin Wng et.al Table 1 of https://arxiv.org/pdf/2209.14278.pdf

[Bes05] eqs above eq.(22) => only if $p>1/2$, we can have $|R^{<}| > 0$.

Say that the bound is meaningful only when $\delta > 2\eps$, Otherwise just randomly guess.

Add corollaries for different models (power query, inverse query, etc.)
